I-SPLIT: Deep Network Interpretability for Split Computing

This work makes a substantial step in the field of split computing, i.e., how to split a deep neural network to host its early part on an embedded device and the rest on a server. So far, potential split locations have been identified exploiting uniquely architectural aspects, i.e., based on the layer sizes. Under this paradigm, the efficacy of the split in terms of accuracy can be evaluated only after having performed the split and retrained the entire pipeline, making an exhaustive evaluation of all the plausible splitting points prohibitive in terms of time. Here we show that not only the architecture of the layers does matter, but the importance of the neurons contained therein too. A neuron is important if its gradient with respect to the correct class decision is high. It follows that a split should be applied right after a layer with a high density of important neurons, in order to preserve the information flowing until then. Upon this idea, we propose Interpretable Split (I-SPLIT): a procedure that identifies the most suitable splitting points by providing a reliable prediction on how well this split will perform in terms of classification accuracy, beforehand of its effective implementation. As a further major contribution of I-SPLIT, we show that the best choice for the splitting point on a multiclass categorization problem depends also on which specific classes the network has to deal with. Exhaustive experiments have been carried out on two networks, VGG16 and ResNet-50, and three datasets, Tiny-Imagenet-200, notMNIST, and Chest X-Ray Pneumonia. The source code is available at https://github.com/vips4/I-Split.

==> tex/discussion.tex <==
\section{Discussion}
\label{cha:discussion}


\todo{Decidere se mantenere la sezione ``Discussion'', oppure scrivere considerazioni varie nei risulatati.} \luigi{Per questo paper, io sarei per commentare tutto nei risultati.}


\iffalse
\subsubsection{Different split point selection approaches}
\federico{questa è una bozza di cosa dovremmo/potremmo dire su questo punto}
One natural objection would be why focus on the saliency, and why the GradCAM algorithm. The saliency of the network is highly dependant on the data the network has been trained on, rather than just the network architecture and structure. This is also evident in the Figure~\ref{fig:CDE_and_fmaps_VGG16}, in which we applied the functional of the Equation \ref{eq:score_func} in the same way we use it to produce the Figure \ref{fig:CDE_and_SEI_VGG16}. As we can see, the isn't a direct comparison between the points identified by both CDE and our approach and the points we could identify directly by the feature maps, in particular at early layers. \federico{help! una motivazione un po' più strong? qualche idea?}

Regarding the GradCAM algorithm, the main difference between other approaches is that combines both the learned information w.r.t. the class predicted and the current information that comes by the feature extractor. \federico{argomentare meglio quel discorso che faceva marco, al momento non riesco a imbandirlo troppo bene}
Furthermore, the GradCAM algorithm is architecture-agnostic thus can be applied at every layer of the network, which is particularly suitable for the task of identify possible split points.

\todo{\federico{Mi serve aiuto per pensare quali altri ablation inserire!!}}
\fi

==> tex/experiments.tex <==
\section{Experimental Results}
\label{cha:experiments}

In this section, we provide an extensive experimental validation of both our claims and the proposed approach.


Since our framework is agnostic with respect to the network architecture, we consider the VGG16 and the ResNet-50 architectures. Other than being the \emph{de-facto} standard for classification, they are also interesting for  split computing; actually, they exhibit a
good base accuracy, a large number of parameters, they are relatively deep in terms of the number of layers, and the dimensionality of the layers has dramatic changes.

We provide results on the Tiny-Imagenet-200 dataset \cite{le2015tiny}, a compact version of ImageNet that comprises a subset of 200 classes, with a training set of 100.000 images, a validation, and a test set of 10.000 images each. All images are 64$\times$64 pixels. \three{We also provide experiments on other two datasets, notMNIST \cite{notMNIST}, and Chest X-Ray Pneumonia \cite{chest_xray}, to demonstrate the strength of our method on datasets with only a few classes (notMNIST), or unbalanced (X-Ray). Due to the page limit, we add these experiments to the Supplementary Materials.}
% \franz{Direi di rimuvere la frase seguente.} We wanted to adopt the same dataset as Sbai et al. \cite{sbai2021cut} for reference, but the dataset has been removed from the online sources. Therefore, without information on the adopted classes and training subdivision, we focused on Tiny-Imagenet-200 which is a public subset of ImageNet with a sufficient number of classes.


We used the PyTorch~\cite{paszke2019pytorch} implementation of the model that was pre-trained on the whole ImageNet data (1000 classes). 
%The bottleneck we used in the experiments is a convolutional autoencoder under-complete formed by an encoder-decoder structure. 
For the bottleneck, we used a standard convolutional under-complete autoencoder with two convolutional layers with stride 2 for the encoder and two for the decoder, setting the number of filters depending on the desired compression rate.
%The encoder presents two 2D convolutional layers, which apply stride 2 on the feature map, increasing the output filters depending on the required compression rate. The decoder takes as input the output of the encoder and recreates the original input of the encoder using transposed 2D convolutions. 
%The whole compression rate is 90\%, for staying in a range which is suitable for the lowest network capabilities, i.e. below 3G bandwidth.
%To simulate realistic communication constraints, we decided to keep constant the amount of data transferred throughout the network, i.e. the number of elements in the bottleneck layer.
%\franz{questo punto è un po' tricky perchè non teniamo costante il rapporto di compressione ma in realtà nemmeno il numero di elementi... dobbiamo trovare un modo convincente per descrivere questa parte.}
For a fair comparison among layers of different dimensionality, we keep constant the compression rate to 90\%, which means that the dimensionality of the encoded data is 10\% of the dimension of the splitting layer.


For the training of the bottleneck, we ran up to 200 epochs with a learning rate of $5\times 10^{-3}$ using the Adam optimizer \cite{kingma2014adam}. Fine-tuning the whole network on 200 classes required up to 100 epochs with a learning rate of $1\times10^{-4}$.


%In the remaining of this section we will validate all our claims; additional experiments, including qualitative results, will be available in the supplementary material.


\subsection{Splitting point selection}
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{img/CDE_and_SEI_VGG16_v2.png}
\end{center}
\caption{Candidate splitting points identified by CDE~\cite{sbai2021cut} and \sei on the VGG16. Local minimum points of CDE correspond to local maximum points of \sei. The red-star markers are two extra points that our \sei method is able to identify. (*) represents a max-pooling layer.}
\label{fig:CDE_and_SEI_VGG16}
\end{figure}


A preliminary goal of our work is to select a set of candidate splitting points that are worth to be deeply analyzed to find the optimum. In this sense, we compare our selection with the candidate points selected by the CDE approach~\cite{sbai2021cut} which is the state of the art in this field. Other approaches cited in Section~\ref{cha:related} are not directly comparable with our \sei since they introduce in the selection phase considerations about the data transmission speed that we decided to ignore in this paper.
Fig.~\ref{fig:CDE_and_SEI_VGG16} shows the results of the selection phase obtained by both (\sei and CDE) methods on the VGG16 architecture. We can clearly appreciate how our method identifies all candidate splitting points output by CDE (namely layers $5$, $9$ and $13$, corresponding to \emph{block2\_pool}, \emph{block3\_pool} and \emph{block4\_pool} respectively), and two additional points at layers $11$ and $15$, corresponding to \emph{block4\_conv2} and \emph{block5\_conv2}.
Indeed, the layers identified by both methods are related to max-pooling layers in the VGG architecture, which are worth conveying more information-per-pixel since there is a local dimensionality reduction with limited loss of information. 
Nevertheless, it is worth noting how layers with the same dimensionality --\ie convolutional layers belonging to the same block-- do not express the same importance as shown by the \sei curve. In these regions of uniform dimensionality, we select layers that have higher importance, and we will show that the \cui values directly translate into higher classification accuracy.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{img/F1_pre_post_VGG16_tiny200_v2.png}
\end{center}
\caption{\three{Behavior of \sei on preserving the per-class performance before the split (\emph{original model}, in blue) and after the split (\emph{split model}, in orange). As expected, no dramatic changes in the single performance are visible, especially with the best and worse performing classes: the best performance does not become the worst after the split, and viceversa.}}
\label{fig:f1_exp}
\vspace{-.8em}
\end{figure}

%\three{As for the balance of performance that different classes may have with the original network, and how this balance may change after the \sei procedure, we present an additional experiment, whose results are reported in Fig.~\ref{fig:f1_exp}. After the training of the original VGG network, we rank the 200 classes in descending F1 order (the blue line). As visible, the performance is unbalanced, since the F1 score ranges from a few decimals to 87\%. Then, the split version driven by the \sei curve is re-trained, and the new F1 scores associated with the classes are reported by the orange line. The plot is very interesting: actually, classes that were best or worst performing \emph{before the split} do not change seriously their performance after the split. For classes with an average performance, the split shuffled a little the F1 scores. Overall, a certain degree of variability is expected, since we showed that for specific classes the best point of split may be different.}
\three{In Fig.~\ref{fig:f1_exp} we show that our method is independent on the performance of the network on specific classes. Here we report the F1 score for all the 200 classes: we can clearly see that the general trend remains after splitting at the best splitting point and retraining with the proposed approach. It is worth noting that a certain degree of variability is expected, since we showed that for some classes this is not the best point of split.}


\subsection{Importance as a proxy for classification accuracy}
\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{img/SEI_and_accuracy_and_grad_boxplot_VGG16_v2.png}
\end{center}
\caption{\two{Classification accuracy achieved when splitting the VGG16 into all the candidate points identified by \sei, compared with the \sei curve (in yellow) and the \emph{Gradients} curve (in gray). (*) represents a max-pooling layer.}}
\label{fig:SEI_and_accuracy_boxplot_VGG16}
\end{figure}


In Fig.~\ref{fig:SEI_and_accuracy_boxplot_VGG16} we report on the same graph results in terms of cumulative importance (\cui) and classification accuracy when splitting the DNN in correspondence of the candidate splitting points identified with \sei. We can clearly see that these results confirm our claim that \cui is a good proxy for classification accuracy. As a result, we confirm that splitting the DNN at layer $15$ is optimal for preserving accuracy.
While the absolute values on classification accuracy are relatively close to each other, we provided a statistical analysis generating 15 testing sets by randomly sampling 800 images from the validation set.
Box plots in Fig.~\ref{fig:SEI_and_accuracy_boxplot_VGG16} demonstrate how the distributions are well separated, and thus the relatively small improvement in accuracy is indeed statistically relevant.

\two{Also, always in Fig.~\ref{fig:SEI_and_accuracy_boxplot_VGG16} we report the result obtained with \emph{Gradients}, the other approach that together with \gradcam passes the ``sanity check'' of \cite{adebayo2018sanity}. As visible, \gradcam gives a better curve in terms of proportionality w.r.t. the final class-accuracy, while \emph{Gradients} is growing as soon as the layer is deeper, making hard to spot the best split point. In particular, the \emph{Gradients} approach brings to a \cui curve whose values are increasing as soon as the layer is deeper. This is due to the vanishing gradient effect: gradients are much higher when closer to the network's end. For this reason, we prefer \gradcam, since the multiplication of the gradients by the values of the feature (close to 0) provides a more constrained range of \cui values. }




\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{img/SEI_and_accuracy_per_dimensionality_VGG16_v2.png}
\end{center}
\caption{Classification accuracy achieved when splitting the VGG16 on all the last four convolutional layers, compared with the \sei curve. (*) represents a max-pooling layer.}
\label{fig:SEI_and_accuracy_per_dimensionality_VGG16}
\end{figure}


To further validate the selection of layer $15$ as the best choice, we explored the behavior of the network on the last four convolutional layers, \ie layers with the same feature dimensionality. 
Results are reported in Fig.~\ref{fig:SEI_and_accuracy_per_dimensionality_VGG16}. 
Again, we can support our decision in selecting layer $15$ over all the other convolutional layers in \emph{block5}. This analysis also validates our claim that the overall accuracy of the network, and thus the best splitting point as defined in this study, cannot only rely on topological aspects of the network architecture --on which all these points are equivalent-- but should also account for our importance-related \textsc{CUI}s.


\subsection{Class-dependent splitting point selection}
\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{img/SEI_and_accuracy_per_class_1and2_VGG16_v2.png}
\end{center}
\caption{Comparison of splitting results for different subsets of classes. Top: \sei curve computed on two different subsets of 15 classes for the last four convolutional layers of the VGG16 architecture. Bottom: classification accuracy for two models trained on the same subsets of 15 classes on layers $13$ and $15$. (*) represents a max-pooling layer.}
\label{fig:SEI_and_accuracy_per_class_1and2_VGG16}
\end{figure}


In this work, we also claim that different subsets of classes can lead to different selections of the best splitting point. To validate this claim we analyzed the \sei curve for each class separately and we identified two different behaviors in the last portion of the network. In particular, when referring to \emph{block5}, we saw that most of the classes achieved a higher \cui at layer $15$, while 15 classes had a global maximum at layer $13$ (see Fig.~\ref{fig:SEI_and_accuracy_per_class_1and2_VGG16}-top). We investigated this phenomenon generating two alternative models by splitting the network into both points, and then retraining these models with two subsets of 15 classes, one for each different behavior. Results, shown in Fig.~\ref{fig:SEI_and_accuracy_per_class_1and2_VGG16}-bottom, demonstrate that the same shape of the \sei curve translates to the accuracy curve. %\franz{commentare nelle conclusioni che si sceglie il punto di split in base alle classi attese.}


\subsection{Extension to ResNet-50}
%\todo{Argomentare i risultati della ResNet-50.}

We ran the same experiments also on the ResNet-50 architecture~\cite{he2016deep}. Results, shown in Fig.~\ref{fig:CDE_and_SEI_ResNet50} are coherent with the ones on VGG16 presented so far. The main difference is the fact that in this case, the \sei curve is smoother, with local maxima located on the max-pooling layers. This is due to the residual structure of the network, which encourages to distill features in a smoother way throughout the entire network. Indeed, not only the \cui is almost constant in layers with the same features dimensionality, but it is also relatively uniform between different blocks. On the other, hand Fig.~\ref{fig:CDE_and_SEI_ResNet50} confirms that \cui is a good proxy for the overall classification accuracy and thus it is worth splitting the network on the global maximum of \sei.


\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{img/CDE_and_SEI_and_accuracy_ResNet50_v3.png}
\end{center}
\caption{Results of the CDE, \sei, and accuracy
on the ResNet-50. The plotted lines show the fit achieved by the two methods. In particular, the local minimum points of CDE correspond to the local maximum points of \sei. The ``star'' marker shows the extra point that is able to identify our method.}
\label{fig:CDE_and_SEI_ResNet50}
\end{figure}

% Nel paper, prima, c'erano queste due qui.
\iffalse
\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{img/CDE_and_SEI_ResNet50.png}
\end{center}
\caption{Results of the CDE and \sei
on the ResNet-50. The plotted lines show the fit achieved by the two methods. In particular, the local minimum points of CDE correspond to the local maximum points of \sei. The ``star'' marker shows the extra point that is able to identify our method.}
\label{fig:CDE_and_SEI_ResNet50}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{img/SEI_and_accuracy_ResNet50.png}
\end{center}
\caption{Accuracy analysis when splitting the ResNet-50 into all the layers, compared with the \sei curve.}
\label{fig:SEI_and_accuracy_ResNet50}
\end{figure}
\fi



==> tex/intro_v01.tex <==
\section{Introduction}
\label{cha:intro}

\iffalse
\franz{Outline:
\begin{itemize}
\item Deep Neural Networks are performing very well in several tasks but are too resource demanding to run on edge devices
\item one way is to simplify the network, and thus decrease accuracy, the other way is to send all the data to the server, and thus have high latency, ...
\item the third way is to split computation across nodes (Franco, can we say this is even more important in 5G where we can split computation across intermediate nodes as well?)
\item recent works propose strategies to identify the best splitting point based on the analysis of the topology of the neural network
\item we claim that the splitting point is not only a function of the network architecture, but should take into account the data processed by the network
\item we propose to use a data visualization technique (GradCam) to estimate the amount of information encoded in each layer of the DNN and select the splitting point as the layer with the highest value
\end{itemize}}
\fi
In the last decade, Deep Neural Networks (DNNs) achieved state-of-the-art performance in a broad range of problems. However, DNN models often present computational requirements that cannot be satisfied by most of the resource-constraint edge devices available today~\cite{matsubara2021split}. This prohibits the full deployment of DNN-based applications on these devices, the \emph{mobile-only} approaches.
In this sense, the most common deployment approach of DNN-based applications on resource-constraint devices is the \emph{cloud-only} approach. With this approach, the network is running on the server-side, and the input is directly transferred from the acquisition device to the server through a network connection. Then, the server computes the inferences and the output is sent back to the device. Using this approach ensures total system accuracy, but the complete transfer of data may lead to an excessive end-to-end delay in degraded channel conditions, and erasure of the task in extreme conditions.

As a compromise between the mobile-only and the cloud-only approaches, recently proposed \emph{split computing} (SC) frameworks ~\cite{shao2020bottlenet++,sbai2021cut,matsubara2022supervised} propose to split DNN models into a head and a tail, deployed at the mobile device and server respectively. Using SC, the computational load is distributed across the mobile device and the server, while also resulting in a lower amount of data to be transferred on the network. In particular, early implementations of SC, such as~\cite{kang2017neurosurgeon}, select a layer $l$ and divide the model in order to define the head and tail submodels. Whereas, more recent SC frameworks introduce the notion of bottleneck to achieving in-model compression toward the global task~\cite{matsubara2019distilled}. After having individuated a split point, and injected a bottleneck to compress and send the data across between head and tail, the whole network needs to be retrained, to define the weight of the bottleneck part (usually, an autoencoder [ref]) and to optimize in general the whole architecture with respect to the final classification performance [ref].
Defining the point of split in a given architecture represents the most problem in the split computing literature nowadays. In the recent~\cite{matsubara2022supervised}, purely architectural considerations drive the decision where to split. The idea is to locate right after max-pooling layers since they downsample feature maps eliminating features with a very low probability of being active~\cite{boureau2010theoretical}. This permits to compress and send between head and tail relevant data only.  Unfortunately, the effectiveness of a split location can be appreciated only after the re-training of the network, since the current splint point conditions are not predictive in the theory of the final performance of the network. On a standard VGG16 network, this means to spend 6 hours to apply the split and evaluate the obtained system.\\

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=\linewidth]{img/Schema.png}
  \end{center}
  \caption{Graphic representation of the \emph{split computing} paradigm. The Deep Neural Network architecture is divided in a \emph{head} part, running on the edge device, and a \emph{tail} part running on a server machine. Intermediate data representation is sent through a network connection after a compression stage.\marco{non va bene, questo deve essere il teaser}}
  \label{fig:Schema}
\end{figure}

In this paper, we propose two main advancements toward a principled way to find the optimal split location for a generic deep network. The former advancement considers the concept of ``importance'' of a neuron~\cite{selvaraju2017grad}, intended as its capability of creating strong gradients with respect to the decision toward a specific class, for specific image input. The famous \emph{grad-cam approach}, given a trained model, an image. and the right class, provides an image map showing which pixels of the image are important for deciding the correct class. This idea can be applied to the feature map provided by each layer of a network, and, after sufficient statistics over test images and classes, it is enough to individuate in general how much the neurons of a layer are crucial for deciding any correct class. A layer that contains a high proportion of important neurons has to be preserved, and a split has to be computed where this percentage is lower. This idea brings to what we dub Split-et-Impera (SeI) system, for deciding automatically a suitable split location. In practice, SeI brings to a 1D plot (see Fig. XX), where the height of each point is a surrogate of the importance of the neurons of that layer. Splitting a network after an important layer guarantees that all the information used until decisive neurons supporting high accuracy is preserved. The higher is the SeI curve, the higher is the accuracy that a network if preserved until that layer, is capable to express. This permits, with just the SeI curve, to have an idea of the performance of the network when different split points will be applied, with the crucial difference of a consistent time saving: a SeI point needs 15 minutes to be computed, versus the 6 hours needed to apply a split and retrain and test a VGG16 network. 
Furthermore, whereas previous studies indicate split candidates as local minima in the size of the layers, SeI is capable of discriminating among layers of the same size, isolating within a plateau of layers of the same size the very best split point.

The second advancement comes directly from the main idea of SeI: if a layer is important in the measure of how decisive are the neurons in deciding any given class, we can specialize this importance to a specific subset of classes, and find different split points depending on the classes which we are more interested in. This provides the fresh-new concept of \emph{class-dependent split decision}, which brings us to decide different split points if our network has to work in a domotic scenario, as in the case of parking (e.g., ``sock'', ``remote control''), or in an outdoor urban scenario, where different classes are more probable (e.g., ``moving van'', ``trolley coach'').
Experiments have been conducted on two of the most popular general-purpose classification networks, the VGG16 \cite{simonyan2014very} and ResNet-50 \cite{he2016deep} confirming each of the claims discussed above, surpassing previous, more empirical justifications as in~\cite{matsubara2022supervised}.\\

Summarizing, the present paper advances in the split computing field in the following ways:
\begin{itemize}
\item Providing SeI, a technique which indicates where to split a deep network in order to preserve the capability of providing high accuracy in the context of image classification
\item SeI is capable of discriminating between network layers of the same size to find the best split point, while previous body of work does not.
\item with SeI, we demonstrate that a split point depend on the classes a classifier has to decide upon, i.e., different classes to be evaluated bring to different split points even if the network architecture is the same. This is a totally new aspect in the literature of split computing
\item SEI is definitely faster that testing a split network post-hoc, going from several hours to few minutes to have a reliable prediction of the accuracy performance of the split network
\item Code and data is available here:
\end{itemize}

%The core contribution of this paper is a novel approach guided by network interpretability~\cite{olah2018building} to identify a set of candidate points where to split DNN models in order to minimize the accuracy loss due to the data compression. This, because, in order to build trust in intelligent systems and move towards their meaningful integration into our everyday lives, we must determine which feature in our inputs affect the final decision of the network. Specifically, using GradCAM technique~\cite{selvaraju2017grad} we analyze the gradients to check on which our model focuses on generating a certain prediction. Based on this result, we can choose the best splitting point of a specific network, in order to improve the overall accuracy.

%In summary, the main contributions of this paper are as follows:
%\begin{itemize}
%  \item We propose a the Split-Et-Impera framework (SEI) framework that, driven by the analysis of class activation maps, identifies the best splitting point for a generic DNN architecture in order to minimize the drop in accuracy for the defined task;
%  \item Through a detailed analysis of two popular network architectures, we demonstrate that the best splitting point is strongly influenced by the input data, rather than only dependent from the network architecture;
%  \item we propose a lossy compression-aware training method to compensate for the accuracy loss.
  %\item The Split-Et-Impera framework (SEI), compared to the Sbai et al. \cite{sbai2021cut} approach, is able to identify more split points and in particular find the optimal points w.r.t. the accuracy of the network for solving the task.
%\end{itemize}

The remainder of the paper is organized as follows. In Section~\ref{cha:related} a state-of-the-art on different split computing frameworks is given. In Section~\ref{cha:method}, we present the core contribution of this paper: a DNN splitting strategy based on class activation maps to maximize offloading performance, and afterward experiments are shown in section Section~\ref{cha:experiments}. Section~\ref{cha:conclusion} concludes the paper.


\section{Previous Related Work section}
\label{cha:related_prev}

In this section, we provide an overview of existing state-of-the-art split computing approaches, combining the discussion regarding different methods of interpretability for neural networks. Relevant literature has been surveyed in~\cite{matsubara2021split} and~\cite{olah2018building} respectively.

\subsection{Split Computing}
%The Split Computing (SC) technique is contextualized in a system composed of a resource constraint device and a server that operate on a DNN model, interconnected via a network channel. For the purpose of this paper, we can distinguish two main trends of related work: without DNN alteration and with bottleneck injection.
Split computing refers to the problem of running a deep learning model on two separate devices, dividing the neural network architecture in two portions and passing data through a network connection.
%We can distinguish two main families of approaches: with and without network alteration.
%
%\luigi{Questa sezione la ridurrei dato che il nostro approccio, rispetto allo stato dell'arte, si colloca nella  subsubsection 2 e non 1.}
%
%\subsubsection{Split Computing without DNN modification} 
%These methods aim at finding the best splitting point for a DNN without allowing to modify the network structure in any way. 
The main goal of split computing methods is to find the best splitting point for a specific  architecture, where the definition of ``best splitting point'' is not shared, as it can be related to minimizing latency and/or energy consumption, or maximizing the overall prediction accuracy. Preliminary works showed that: 
(1) neither cloud-only or mobile-only approaches are  optimal~\cite{eshratifar2019jointdnn};
(2) splitting in the first layers is beneficial for speeding up computation, while splitting in the last layers allow to preserve higher performances~\cite{kang2017neurosurgeon}; and
(3) latency can be reduced without significant drop in accuracy by either neural network quantization~\cite{li2018auto} or lossy compression before data transmission~\cite{choi2018deep,cohen2020lightweight}.

%Kang et al. \cite{kang2017neurosurgeon} designed ``Neurosurgeon'', a lightweight scheduler to automatically partition DNN computation for minimizing total latency and energy consumption. Their evaluations show that the most suitable splitting layers to optimize latency and energy consumption are the input layers of the models. Starting from this work, the scientific community started to conduct a study on the best split computing techniques, mainly focused on tasks such as image classification.

%In \cite{li2018auto}, Li et al. proposed an auto-tuning neural network quantization framework for cloud-edge collaborative inference. For each neural network tested, the framework gives the best partition point and the fastest partition point. In addition, they have shown that quantized neural networks do not lead to a significant drop in accuracy (usually less than 1\%).

%Eshratifar et al. \cite{eshratifar2019jointdnn} propose an efficient, adaptive, and practical engine, called ``JointDNN'', for cloud-edge collaborative inference. They showed that the cloud-only or mobile-only approaches are not optimal concerning latency and energy consumption.

%Choi and Bajic in \cite{choi2018deep} showed that the efficiency of a cloud-edge collaborative inference can be further improved by lossy compression of feature data. Experiments indicate that using this strategy, the communication overhead can be reduced by up to 70\% without sacrificing accuracy.

%In \cite{cohen2020lightweight}, Cohen et al. present a novel lightweight compression technique designed specifically to code the activations of a split DNN layer while having a low complexity suitable for edge devices and not requiring any retraining.

%From all these works, we can see that communication delay to transfer data from a low-complexity device to the server is a key component in SC to reduce the latency.


%\subsubsection{Split Computing with bottleneck injection}\label{sota:bottleneck}
%For the reason mentioned above, introducing artificial bottlenecks to DNN models can allow us to minimize total inference time in a SC scenario. As mentioned in \cite{matsubara2021split}, \cite{eshratifar2019bottlenet} and \cite{matsubara2019distilled} were the first to propose altering existing DNN architectures through the use of bottlenecks at early layers in DNN models so that communication delay (cost) and total inference time can be further reduced.

%In \cite{hu2020fast}, Hu and Krishnamachari proposed a streaming inference framework to simultaneously improve throughput and accuracy by communication compression.

%Jankowski et al. \cite{jankowski2020joint} proposed an autoencoder-based network for intermediate feature map transmission to allow bandwidth reduction.

Based on these findings, many different criteria have been proposed in the literature to find the best splitting point and compress data for transmission over the network.
Many authors proposed to use an autoencoder structure as a bottleneck for intermediate feature map transmission to reduce the communication delay and thus the total inference time~\cite{matsubara2019distilled,eshratifar2019bottlenet,jankowski2020joint}, while other approaches try to find a good compromise between throughput and accuracy~\cite{hu2020fast}. 
In this sense, recent works provided a discussion on the trade-off between the model inference accuracy and the averaged compression ratio of offloaded data~\cite{yao2020deep} and between accuracy and memory size on mobile devices, considering communication constraints
based on different protocols~\cite{sbai2021cut}. More recent works are also trying to further improve the overall inference time by modifying the network structure deployed to the edge device by using knowledge distillation training the network with a teacher-student approach~\cite{matsubara2021supervised}.
\franz{non ho capito quale sia il main contribution di~\cite{matsubara2021neural}.}
%In \cite{matsubara2021neural}, Matsubara and Levorato modify the architecture of the network to achieve in-network compression by introducing a bottleneck layer in the early layers. Also, Matsubara et al. in \cite{matsubara2021supervised}, adopt the ideas from knowledge distillation and neural image compression to compress intermediate feature representations more efficiently to obtain better-supervised rate-distortion performance while maintaining smaller end-to-end latency.
While the introduction of a bottleneck structure is necessary to avoid overload on the network channel, the main limitation of all these methods is related to the selection of the splitting point. Indeed, all these works assume that the best splitting point is related exclusively to the topology of the neural network architecture, selecting points that are inevitably related to max pooling layers, \ie local minima in feture map dimensionality. 
\ul{In this paper we demonstrate that, keeping constant the amount of data transmitted on the network channel, best accuracy results are achieved by splitting at the layer that has the highest activation of the feature maps.} \franz{da rivedere, scritta male!}

==> tex/intro_v02.tex <==
\section{Introduction}
\label{cha:intro}


%\todo{Decidere se utilizzare ``split'' o ``splitting'' point, e poi uniformare in tutto il paper.} \luigi{Per ora, ho uniformato tutto con ``splitting''.}


In the last decade, Deep Neural Networks (DNNs) achieved state-of-the-art performance in a broad range of problems. However, the DNN computational requirements preclude their deployment on most of the resource-constraint devices, such as mobile phones, available today~\cite{matsubara2021split}; we refer to this scenario as \emph{device-only}. A possible alternative is to run simplified models on the devices~\cite{sandler2018mobilenetv2}, but this has an impact on the overall accuracy, which may not be desirable. The current approach, usually referred to as \emph{cloud-only}, is to transfer the data captured by the device to a server through a communication network. The servers, which run the DNN model, compute the inference and send it back to the device. 
%In this scenario, the overall inference time depends, in addition to the model processing time, on the data transfer time. In case of degraded transmission channel conditions, this may lead to an excessive end-to-end delay.
In this scenario, the overall inference time depends, in addition to the model processing time, on the data transfer time which may lead to an excessive end-to-end delay.

As a compromise between the device-only and the cloud-only approaches, the \emph{split computing} (SC) frameworks~\cite{shao2020bottlenet++,sbai2021cut,matsubara2022supervised} propose to divide DNN models into a ``head'' and a ``tail'', deployed at the edge device and at the server, respectively. 
While this has an impact on the processing time, in order to decrease the impact of the transfer time, the splitting point is chosen such that the amount of data to be transferred is less than the input data that would be transferred in a cloud-only scenario. Early implementations of SC, such as~\cite{kang2017neurosurgeon}, relied on the characteristics of the DNN (dimensions of each layer), with no modifications. Nevertheless, for a given DNN architecture, the split points are limited. Recent SC frameworks introduce the notion of \emph{bottleneck injection}. Given a layer, an additional structure, such as an autoencoder, is inserted to achieve in-model compression~\cite{matsubara2019distilled}.
\hl{x Franco: puoi inserire qui una frase o due che motivino che questo approccio avr\`a ancora pi\`u impatto con l'avvento del 5G?}


The bottleneck introduces a trade-off: on the one hand, a higher compression decreases the transmission time, on the other hand, such compression is lossy and it may have a strong impact on the overall accuracy. So far, this trade-off has been explored using purely architectural considerations. For instance, in~\cite{sbai2021cut}, the authors first locate the potential splitting layers by focusing on the max-pooling layers -- such layers, in fact, downsample feature maps eliminating features with a very low probability of being active~\cite{boureau2010theoretical}. After that, they fine-tune the bottleneck characteristics to improve the overall accuracy. This approach requires a trial-and-error cycle that may be time-consuming -- on a standard VGG16 network, the evaluation of a single split point may take up to six hours on commodity hardware. Some architectures, for instance, may have a series of layers with equal sizes after a max-pooling layer, so it is not clear where to optimally split the model.


\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{img/Figure_1.png}
\end{center}
\caption{Graphic representation of the \emph{split computing} paradigm. The Deep Neural Network architecture is divided into a \emph{head} part running on the edge device, and a \emph{tail} part running on a server machine. Intermediate data representation is sent through a network connection after a compression stage. \marco{non va bene, questo deve essere il teaser} \franz{a me adesso piace}}
\label{fig:Schema}
\end{figure}


\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{img/Figure_2.png}
\end{center}
\caption{Overview of our one-shot framework \sei{}. The input images are fed into a neural network. Then, we extract high-resolution saliency maps through the use of the \gradcam{} algorithm for each layer. At this point, for each $i$-th layer of the network, we mediate among each other all the maps of each image of each class. Finally, we evaluate each map at each $i$-th layer to define the yellow curve, where we identify local maxima.}
\label{fig:Figure_2}
\end{figure*}


In this paper, we propose a principled way of finding the optimal split location for a generic DNN. To this aim, we consider not only the layer sizes but also how much information is encoded in each layer, identifying the layers that are more robust to the introduction of a bottleneck. In particular, we consider the \emph{\gradcam{} approach}~\cite{selvaraju2017grad} that relies on the concept of ``importance'' of a neuron~\cite{selvaraju2017grad}, \ie its capability of creating strong gradients with respect to the decision toward a class, for specific input.  In the case of image classification, given a trained model, an image, and its class, \gradcam{} provides an image map showing which pixels of the image are important for deciding the correct class. This process can be repeatedly applied to the feature map of each DNN layer using a set of test images in order to identify, in general, how much the neurons of a layer are crucial for deciding any correct class. A layer that contains a high proportion of important neurons is more robust and presents a suitable point for a split.
% [IT WAS:] A layer that contains a high proportion of important neurons has to be preserved, and a split has to be computed where this percentage is lower.


In our approach, which we call \emph{Split-et-Impera} (\sei{}), we compute the aggregated importance for each layer, which is then used as an indication of the impact on the accuracy of a split in that layer. There are different advantages offered by \sei{}. The process is computationally efficient and can be done in a few minutes, instead of hours as done with the trial-and-error approach. \franz{questo claim \`e forzato, valutiamo come metterlo.} 
In addition, we are able to discriminate, in the case of layers with the same size, which one is best suitable as a split point. Finally, we can adapt the computation using different inputs. This last benefit is particularly interesting: for a given DNN, we can specialize the computation of the importance of each layer using a specific subset of classes, and find different split points depending on different subsets. This provides the fresh-new concept of \emph{class-dependent split decision}, which allows us to adapt the split point depending on the context of use.


Our experiments conducted on two of the most popular general-purpose classification networks --VGG16 \cite{simonyan2014very}, and ResNet-50 \cite{he2016deep}-- confirm each of the claims discussed above, surpassing previous, more empirical justifications as in~\cite{sbai2021cut}. In summary, this paper advances in the split computing field in the following ways:
%
\begin{itemize}
\item We identify a principle way, based on the concept of neuron importance, to analyze a DNN and find suitable split points that preserve the capability of providing high accuracy in the context of image classification;
\item We implement such approach in a tool, called \sei{}, that is computationally faster than the state-of-the-art approaches in identifying  the optimal split point;
\item With \sei{}, we are able to determine different split points based on the classes a classifier has to decide upon.
\end{itemize}

The remainder of the paper is organized as follows. In Section~\ref{cha:related} we review the literature on split computing. In Section~\ref{cha:method}, we present the core contribution of this paper: a DNN split strategy based on class activation maps to maximize offloading performance. We show the experimental results in Section~\ref{cha:experiments}, while Section~\ref{cha:conclusion} concludes the paper. The code and the data will be available upon acceptance of the paper. %here: \url{http:\\}
